Submillimeter continuum variability in Planck Galactic cold clumps

In the early stages of star formation, a protostar is deeply embedded in an optically thick envelope such that it is not directly observable. Variations in the protostellar accretion rate, however, will cause luminosity changes that are reprocessed by the surrounding envelope and are observable at submillimeter wavelengths. We searched for submillimeter flux variability toward 12 Planck Galactic Cold Clumps detected by the James Clerk Maxwell Telescope (JCMT)-SCUBA-2 Continuum Observations of Pre-protostellar Evolution (SCOPE) survey. These observations were conducted at 850 um using the JCMT/SCUBA-2. Each field was observed three times over about 14 months between 2016 April and 2017 June. We applied a relative flux calibration and achieved a calibration uncertainty of ~ 3.6% on average. We identified 136 clumps across 12 fields and detected four sources with flux variations of ~ 30%. For three of these sources, the variations appear to be primarily due to large-scale contamination, leaving one plausible candidate. The flux change of the candidate may be associated with low- or intermediate-mass star formation assuming a distance of 1.5 kpc, although we cannot completely rule out the possibility that it is a random deviation. Further studies with dedicated monitoring would provide a better understanding of the detailed relationship between submillimeter flux and accretion rate variabilities while enhancing the search for variability in star-forming clumps farther away than the Gould Belt.

==> tab4.tex <==
\begin{deluxetable*}{lcc|rc ccrrr}
\tabletypesize{\scriptsize}
\setlength{\tabcolsep}{0.04in}
\tablecaption{Properties of Comparable ATLASGAL Clumps from \citet{urquhart2018} \label{tab:comp}}
\tablewidth{0pt}
\tablehead{
\colhead{} & \colhead{} && \colhead{$r$\tablenotemark{a}} & \colhead{} &
\colhead{$\vlsr$} &\colhead{} & 
\colhead{$d$} & \colhead{$\Lbol$} & \colhead{$\Mclump$}  \\
\colhead{\#} & \colhead{Outliers} && \colhead{(\arcsec)} & \colhead{ATLASGAL Clumps} & 
\colhead{(\kms)} & \colhead{Phase} &
\colhead{(kpc)} & \colhead{($\Lsun$)} & \colhead{($\Msun$)}
}
%\colnumbers
\startdata
1& G14.143$-$0.508 &&  3 & AGAL014.142$-$00.509    &  21.1 & Quiescent    &  1.5 &   37 &   23 \\
2& G14.210$-$0.598 && 15 & AGAL014.214$-$00.597    &  18.6 & Protostellar &  1.5 &   14 &  137 \\
3& G24.008$+$0.203 &&  3 & AGAL024.009$+$00.202    &  99.3 & YSO          &  7.8 & 1213 &  622 \\
4& G25.635$-$0.126 &&  3 & AGAL025.636$-$00.126    &  93.9 & Protostellar & 10.2 & 1104 & 4581 \\
\enddata                   
\tablenotetext{a}{Angular distance from an outlier to the center of an ATLASGAL clump.}
%		}
\end{deluxetable*}

